Continuous-Time Estimation-Aware Optimal Control of Mobile Sensors for Target Tracking

Target tracking is the problem of estimating the state of a target system using measurements collected (oftentimes) by mobile sensors. Trajectory optimization for mobile sensors must account not only for dynamical and operational constraints, but also for uncertainty in estimating the target system's state. We propose an estimation-aware optimal control method for target tracking that accounts for the nonlinear dynamics of both the mobile sensor and target system, the nonlinear covariance dynamics in extended Kalman filtering, and nonlinear measurement models. Furthermore, it ensures constraints on the mobile sensor are satisfied in continuous time (within numerical precision). In numerical simulations, the proposed method achieves estimation-aware target tracking while satisfying the mobile-sensor constraints in continuous time, even under sparse time discretization.

==> Figures/constaint_violation_plot_10nodes.tex <==
\pgfplotsset{every tick label/.append style={font=\large}}
\begin{subfigure}[t]{.4\textwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        % xlabel = \footnotesize Covariance Objective,
        % ylabel = \footnotesize Energy Objective,
        width = \linewidth,
        height = \linewidth,
        ymin = -0.5, ymax = 1.5,
        xmin = 0, xmax = 10,
    ]
    \addplot [color=case_2_color, line width=1.5pt, forget plot]
    table{%
    0	1
    0.04466778336	1.000149625
    0.08933556672	1.000598313
    0.1340033501	1.001345501
    0.1786711334	1.002390251
    0.2233389168	1.003731252
    0.2680067002	1.005366819
    0.3126744835	1.007294894
    0.3573422669	1.009513051
    0.4020100503	1.012018492
    0.4466778336	1.014808055
    0.491345617	1.017878211
    0.5360134003	1.021225069
    0.5806811837	1.024844381
    0.6253489671	1.028731539
    0.6700167504	1.032881582
    0.7146845338	1.037289203
    0.7593523171	1.041948743
    0.8040201005	1.046854205
    0.8486878839	1.051999253
    0.8933556672	1.057377216
    0.9380234506	1.062981096
    0.9826912339	1.068803569
    1.027359017	1.074836994
    1.072026801	1.081073415
    1.116694584	1.087501016
    1.161362367	1.093833341
    1.206030151	1.09988503
    1.250697934	1.105644957
    1.295365717	1.111102498
    1.340033501	1.116247538
    1.384701284	1.121070484
    1.429369068	1.125562271
    1.474036851	1.129714369
    1.518704634	1.133518792
    1.563372418	1.136968105
    1.608040201	1.140055428
    1.652707984	1.142774446
    1.697375768	1.145119411
    1.742043551	1.147085148
    1.786711334	1.148667061
    1.831379118	1.149861137
    1.876046901	1.150663946
    1.920714685	1.151072649
    1.965382468	1.151084997
    2.010050251	1.150699336
    2.054718035	1.149914606
    2.099385818	1.148730345
    2.144053601	1.147146686
    2.188721385	1.14516436
    2.233389168	1.142784696
    2.278056951	1.140009618
    2.322724735	1.136841644
    2.367392518	1.133283886
    2.412060302	1.129340047
    2.456728085	1.125014416
    2.501395868	1.120311868
    2.546063652	1.115237859
    2.590731435	1.109798419
    2.635399218	1.104000153
    2.680067002	1.097850229
    2.724734785	1.091356378
    2.769402568	1.084526886
    2.814070352	1.077370585
    2.858738135	1.069896848
    2.903405918	1.062115583
    2.948073702	1.054037221
    2.992741485	1.045672711
    3.037409269	1.037033509
    3.082077052	1.02813157
    3.126744835	1.018979339
    3.171412619	1.009589736
    3.216080402	0.9999761523
    3.260748185	0.9901524339
    3.305415969	0.9801328733
    3.350083752	0.9699099343
    3.394751535	0.9592599094
    3.439419319	0.9481177769
    3.484087102	0.9364796178
    3.528754886	0.9243420997
    3.573422669	0.9117024833
    3.618090452	0.8985586284
    3.662758236	0.8849089984
    3.707426019	0.8707526661
    3.752093802	0.8560893173
    3.796761586	0.8409192548
    3.841429369	0.8252434021
    3.886097152	0.8090633055
    3.930764936	0.7923811375
    3.975432719	0.7751996975
    4.020100503	0.7575224142
    4.064768286	0.7393533458
    4.109436069	0.7206971805
    4.154103853	0.7015592364
    4.198771636	0.6819454609
    4.243439419	0.6618624293
    4.288107203	0.6413173436
    4.332774986	0.6203180296
    4.377442769	0.5988729347
    4.422110553	0.5769911247
    4.466778336	0.5547583889
    4.511446119	0.5326386127
    4.556113903	0.5107106379
    4.600781686	0.4889768109
    4.64544947	0.4674394176
    4.690117253	0.4461006833
    4.734785036	0.4249627724
    4.77945282	0.4040277882
    4.824120603	0.3832977726
    4.868788386	0.3627747059
    4.91345617	0.3424605067
    4.958123953	0.3223570318
    5.002791736	0.3024660757
    5.04745952	0.282789371
    5.092127303	0.2633285875
    5.136795087	0.2440853329
    5.18146287	0.225061152
    5.226130653	0.2062575269
    5.270798437	0.1876758768
    5.31546622	0.169317558
    5.360134003	0.1511838638
    5.404801787	0.1332760244
    5.44946957	0.1155952066
    5.494137353	0.09814251431
    5.538805137	0.08091898792
    5.58347292	0.0639724499
    5.628140704	0.0474815523
    5.672808487	0.03146723821
    5.71747627	0.01593305396
    5.762144054	0.0008819219755
    5.806811837	-0.01368385811
    5.85147962	-0.02776260814
    5.896147404	-0.04135326949
    5.940815187	-0.05445540037
    5.98548297	-0.06706917337
    6.030150754	-0.07919537149
    6.074818537	-0.09083538456
    6.11948632	-0.1019912049
    6.164154104	-0.1126654219
    6.208821887	-0.1228612176
    6.253489671	-0.1325823597
    6.298157454	-0.1418331962
    6.342825237	-0.1506186485
    6.387493021	-0.1589442035
    6.432160804	-0.1668159071
    6.476828587	-0.1742403547
    6.521496371	-0.1812246838
    6.566164154	-0.187776565
    6.610831937	-0.1939041914
    6.655499721	-0.1996162704
    6.700167504	-0.2049848275
    6.744835288	-0.2101605462
    6.789503071	-0.2151361679
    6.834170854	-0.219897598
    6.878838638	-0.2244311527
    6.923506421	-0.2287235733
    6.968174204	-0.2327620366
    7.012841988	-0.2365341673
    7.057509771	-0.24002805
    7.102177554	-0.2432322388
    7.146845338	-0.2461357693
    7.191513121	-0.2487281673
    7.236180905	-0.2509994596
    7.280848688	-0.2529401831
    7.325516471	-0.2545413931
    7.370184255	-0.2557946725
    7.414852038	-0.2566921394
    7.459519821	-0.2572264545
    7.504187605	-0.2573908287
    7.548855388	-0.2571790291
    7.593523171	-0.2565853859
    7.638190955	-0.2556047976
    7.682858738	-0.2542327361
    7.727526521	-0.2524652521
    7.772194305	-0.2502989788
    7.816862088	-0.2477814175
    7.861529872	-0.2449910494
    7.906197655	-0.2419282422
    7.950865438	-0.2385927371
    7.995533222	-0.2349846738
    8.040201005	-0.2311045904
    8.084868788	-0.2269534241
    8.129536572	-0.2225325112
    8.174204355	-0.2178435868
    8.218872138	-0.2128887842
    8.263539922	-0.2076706337
    8.308207705	-0.2021920618
    8.352875489	-0.196456389
    8.397543272	-0.1904673283
    8.442211055	-0.1842289828
    8.486878839	-0.1777458428
    8.531546622	-0.1710227833
    8.576214405	-0.1640650606
    8.620882189	-0.1568783086
    8.665549972	-0.1494685353
    8.710217755	-0.1418421177
    8.754885539	-0.1340057985
    8.799553322	-0.1259666803
    8.844221106	-0.1177322211
    8.888888889	-0.1093102283
    8.933556672	-0.1009471255
    8.978224456	-0.09288735135
    9.022892239	-0.0851358463
    9.067560022	-0.07769735175
    9.112227806	-0.07057640834
    9.156895589	-0.06377735431
    9.201563372	-0.05730432428
    9.246231156	-0.0511612477
    9.290898939	-0.04535184758
    9.335566723	-0.03987963935
    9.380234506	-0.03474792948
    9.424902289	-0.02995981464
    9.469570073	-0.02551818046
    9.514237856	-0.02142570064
    9.558905639	-0.01768483613
    9.603573423	-0.01429783417
    9.648241206	-0.01126672769
    9.692908989	-0.008593334537
    9.737576773	-0.006279256887
    9.782244556	-0.004325880758
    9.826912339	-0.002734375483
    9.871580123	-0.001505693385
    9.916247906	-0.0006405694149
    9.96091569	-0.0001395209274
    };
    \addplot [color=case_2_color, only marks, mark size=2pt, mark=*, mark options={solid, fill=case_2_color, draw=case_2_color}, forget plot]
    table{%
    0	1
    1.111111111	1.086690317
    2.222222222	1.143416768
    3.333333333	0.9737777221
    4.444444444	5.66E-01
    5.555555556	0.07451944883
    6.666666667	-0.2009804292
    7.777777778	-0.2500000098
    8.888888889	-0.1093102283
    10	-3.56E-11
    };
    \draw[black, dashed, line width=2.0pt] (0,175) -- (100,175) node[above left]{Maximum};
    \draw[black, dashed, line width=2.0pt] (0,25) -- (100,25) node[below left]{Minimum};
    \end{axis}
    \end{tikzpicture}%
    \caption{LTE example with \(n_k = 10\).}
\end{subfigure}
\begin{subfigure}[t]{.4\textwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        % xlabel = \footnotesize Covariance Objective,
        % ylabel = \footnotesize Energy Objective,
        width = \linewidth,
        height = \linewidth,
        ymin = 0, ymax = 15,
        xmin = 0, xmax = 10,
    ]
    \addplot [color=case_2_color, line width=1.5pt, forget plot]
    table{%
    0	7.071067812
    0.04466778336	7.100978182
    0.08933556672	7.127537815
    0.1340033501	7.150744357
    0.1786711334	7.17059571
    0.2233389168	7.187090045
    0.2680067002	7.200225816
    0.3126744835	7.210001783
    0.3573422669	7.216417031
    0.4020100503	7.219470992
    0.4466778336	7.219163475
    0.491345617	7.215494691
    0.5360134003	7.208465295
    0.5806811837	7.198076413
    0.6253489671	7.184329693
    0.6700167504	7.167227345
    0.7146845338	7.146772192
    0.7593523171	7.12296773
    0.8040201005	7.09581819
    0.8486878839	7.065328607
    0.8933556672	7.031504896
    0.9380234506	6.994353944
    0.9826912339	6.953883698
    1.027359017	6.910103283
    1.072026801	6.863023111
    1.116694584	6.812655851
    1.161362367	6.759080471
    1.206030151	6.702357677
    1.250697934	6.642510784
    1.295365717	6.579565687
    1.340033501	6.51355115
    1.384701284	6.444499129
    1.429369068	6.372445135
    1.474036851	6.297428651
    1.518704634	6.219493593
    1.563372418	6.13868885
    1.608040201	6.055068881
    1.652707984	5.968694408
    1.697375768	5.879633199
    1.742043551	5.78796097
    1.786711334	5.693762411
    1.831379118	5.597132369
    1.876046901	5.498177203
    1.920714685	5.397016341
    1.965382468	5.293784075
    2.010050251	5.188631625
    2.054718035	5.081729514
    2.099385818	4.9732703
    2.144053601	4.863471723
    2.188721385	4.752580298
    2.233389168	4.641021969
    2.278056951	4.532264666
    2.322724735	4.427713957
    2.367392518	4.327430846
    2.412060302	4.231473927
    2.456728085	4.139898456
    2.501395868	4.052755333
    2.546063652	3.970090003
    2.590731435	3.891941292
    2.635399218	3.8183402
    2.680067002	3.749308678
    2.724734785	3.684858415
    2.769402568	3.624989677
    2.814070352	3.569690233
    2.858738135	3.518934416
    2.903405918	3.472682343
    2.948073702	3.430879351
    2.992741485	3.393455668
    3.037409269	3.360326341
    3.082077052	3.331391451
    3.126744835	3.30653659
    3.171412619	3.285633622
    3.216080402	3.268541687
    3.260748185	3.255108418
    3.305415969	3.245171345
    3.350083752	3.238571115
    3.394751535	3.235193256
    3.439419319	3.234718078
    3.484087102	3.23678833
    3.528754886	3.241056941
    3.573422669	3.24718943
    3.618090452	3.254865823
    3.662758236	3.263782093
    3.707426019	3.273651178
    3.752093802	3.284203617
    3.796761586	3.295187868
    3.841429369	3.306370355
    3.886097152	3.317535302
    3.930764936	3.328484403
    3.975432719	3.339036371
    4.020100503	3.349026399
    4.064768286	3.358305582
    4.109436069	3.366740301
    4.154103853	3.37421162
    4.198771636	3.380614691
    4.243439419	3.385858193
    4.288107203	3.389863812
    4.332774986	3.392565777
    4.377442769	3.393910445
    4.422110553	3.393855954
    4.466778336	3.392352178
    4.511446119	3.389261523
    4.556113903	3.38455629
    4.600781686	3.378239338
    4.64544947	3.370324321
    4.690117253	3.360835753
    4.734785036	3.34980917
    4.77945282	3.337291357
    4.824120603	3.323340658
    4.868788386	3.308027363
    4.91345617	3.29143417
    4.958123953	3.273656715
    5.002791736	3.254804177
    5.04745952	3.234999939
    5.092127303	3.214382303
    5.136795087	3.193105246
    5.18146287	3.17133919
    5.226130653	3.149271786
    5.270798437	3.127108651
    5.31546622	3.10507405
    5.360134003	3.083411462
    5.404801787	3.062383979
    5.44946957	3.042274475
    5.494137353	3.023385478
    5.538805137	3.006038655
    5.58347292	2.99050274
    5.628140704	2.976866861
    5.672808487	2.965477616
    5.71747627	2.956721362
    5.762144054	2.95099563
    5.806811837	2.948705382
    5.85147962	2.95025856
    5.896147404	2.956060998
    5.940815187	2.96651081
    5.98548297	2.98199246
    6.030150754	3.002870739
    6.074818537	3.029484928
    6.11948632	3.062143446
    6.164154104	3.101119266
    6.208821887	3.146646344
    6.253489671	3.198917241
    6.298157454	3.258082042
    6.342825237	3.324248568
    6.387493021	3.397483809
    6.432160804	3.477816398
    6.476828587	3.565239944
    6.521496371	3.659716948
    6.566164154	3.761183081
    6.610831937	3.869551586
    6.655499721	3.984717604
    6.700167504	4.106050312
    6.744835288	4.232128903
    6.789503071	4.362693044
    6.834170854	4.497549536
    6.878838638	4.636516594
    6.923506421	4.779423824
    6.968174204	4.926112001
    7.012841988	5.076432701
    7.057509771	5.230247827
    7.102177554	5.387429077
    7.146845338	5.547857374
    7.191513121	5.71142228
    7.236180905	5.87802141
    7.280848688	6.047559861
    7.325516471	6.219949665
    7.370184255	6.395109258
    7.414852038	6.572962994
    7.459519821	6.753440673
    7.504187605	6.936477114
    7.548855388	7.122011757
    7.593523171	7.309988287
    7.638190955	7.500354296
    7.682858738	7.693060973
    7.727526521	7.888062811
    7.772194305	8.085317348
    7.816862088	8.282567756
    7.861529872	8.476219051
    7.906197655	8.666147937
    7.950865438	8.852285116
    7.995533222	9.034568976
    8.040201005	9.212944574
    8.084868788	9.387362786
    8.129536572	9.557779573
    8.174204355	9.724155367
    8.218872138	9.886454536
    8.263539922	10.04464493
    8.308207705	10.1986975
    8.352875489	10.34858592
    8.397543272	10.49428636
    8.442211055	10.63577716
    8.486878839	10.77303867
    8.531546622	10.90605299
    8.576214405	11.03480386
    8.620882189	11.15927649
    8.665549972	11.2794574
    8.710217755	11.39533435
    8.754885539	11.50689621
    8.799553322	11.61413287
    8.844221106	11.71703516
    8.888888889	11.8155948
    8.933556672	11.90981014
    8.978224456	11.99967826
    9.022892239	12.08519014
    9.067560022	12.16633752
    9.112227806	12.24311285
    9.156895589	12.31550925
    9.201563372	12.38352045
    9.246231156	12.44714077
    9.290898939	12.50636506
    9.335566723	12.5611887
    9.380234506	12.61160757
    9.424902289	12.65761798
    9.469570073	12.69921672
    9.514237856	12.73640096
    9.558905639	12.7691683
    9.603573423	12.79751672
    9.648241206	12.82144456
    9.692908989	12.84095054
    9.737576773	12.8560337
    9.782244556	12.86669344
    9.826912339	12.87292947
    9.871580123	12.87474183
    9.916247906	12.87213086
    9.96091569	12.86509723
    10	12.85531559
    };
    \addplot [color=case_2_color, only marks, mark size=2pt, mark=*, mark options={solid, fill=case_2_color, draw=case_2_color}, forget plot]
    table{%
    0	7.071067812
    1.111111111	6.819130402
    2.222222222	4.668861265
    3.333333333	3.240660398
    4.444444444	3.393294092
    5.555555556	2.999999999
    6.666666667	4.014557543
    7.777777778	8.110130554
    8.888888889	11.8155948
    10	12.85531559
    };
    \draw[black, dashed, line width=2.0pt] (0,30) -- (100,30) node[below left]{Minimum};
    \end{axis}
    \end{tikzpicture}%
    \caption{UAV-UGV example with \(n_k = 10\).}
\end{subfigure}

==> related/related.tex <==
\section{Related Work}
